Learning Rich Representations For Structured Visual Prediction Tasks

We describe an approach to learning rich representations for images, that enables simple and effective predictors in a range of vision tasks involving spatially structured maps. Our key idea is to map small image elements to feature representations extracted from a sequence of nested regions of increasing spatial extent. These regions are obtained by "zooming out" from the pixel/superpixel all the way to scene-level resolution, and hence we call these zoom-out features. Applied to semantic segmentation and other structured prediction tasks, our approach exploits statistical structure in the image and in the label space without setting up explicit structured prediction mechanisms, and thus avoids complex and expensive inference. Instead image elements are classified by a feedforward multilayer network with skip-layer connections spanning the zoom-out levels. When used in conjunction with modern neural architectures such as ResNet, DenseNet and NASNet (to which it is complementary) our approach achieves competitive accuracy on segmentation benchmarks. In addition, we propose an approach for learning category-level semantic segmentation purely from image-level classification tag. It exploits localization cues that emerge from training a modified zoom-out architecture tailored for classification tasks, to drive a weakly supervised process that automatically labels a sparse, diverse training set of points likely to belong to classes of interest. Finally, we introduce data-driven regularization functions for the supervised training of CNNs. Our innovation takes the form of a regularizer derived by learning an autoencoder over the set of annotations. This approach leverages an improved representation of label space to inform extraction of features from images

==> diagrams/include/blobs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Blobs.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Draw blob (back).
% Arguments:
% #1 x-size
% #2 y-size
% #3 z-size
% #4 style
\newcommand{\drawBlobBack}[4]{
   \ThreeDput[normal=1 0 0](0,0,0){
      \psframe[style=#4,fillcolor=white](#1,#2)}   % back
   \ThreeDput[normal=0 1 0](#3,#1,0){
      \psframe[style=#4,fillcolor=white](#3,#2)}   % far side
   \ThreeDput[normal=0 0 1](0,0,0){
      \psframe[style=#4,fillcolor=white](#3,#1)}   % bottom
}

% Draw blob (front).
% Arguments:
% #1 x-size
% #2 y-size
% #3 z-size
% #4 style
\newcommand{\drawBlobFront}[4]{
   \ThreeDput[normal=0 0 1](0,0,#2){
      \psframe[style=#4](#3,#1)}                   % top
   \ThreeDput[normal=0 1 0](#3,0,0){
      \psframe[style=#4](#3,#2)}                   % near side
   \ThreeDput[normal=1 0 0](#3,0,0){
      \psframe[style=#4](#1,#2)}                   % front
}

% Draw blob.
% Arguments:
% #1 x-size
% #2 y-size
% #3 z-size
% #4 style
\newcommand{\drawBlob}[4]{
   \drawBlobBack{#1}{#2}{#3}{#4}
   \drawBlobFront{#1}{#2}{#3}{#4}
}

% Draw blob with hypercolumn line.
% Arguments:
% #1 x-size
% #2 y-size
% #3 z-size
% #4 blob style
% #5 hc x-coord
% #6 hc y-coord
% #7 hc style
\newcommand{\drawBlobHC}[7]{
   \drawBlobBack{#1}{#2}{#3}{#4}                   % blob back
   \ThreeDput[normal=1 0 0](0,#5,#6){              % intersection back
      \psdot[dotsize=1.0](0,0)
   }
   \ThreeDput[normal=0 -1 0](0,#5,#6){             % hypercolumn
      \psline[style=#7]{-}(0,0)(#3,0)
   }
   \drawBlobFront{#1}{#2}{#3}{#4}                  % blob front
   \ThreeDput[normal=1 0 0](#3,#5,#6){             % intersection front
      \psdot[dotsize=1.0](0,0)
   }
}

% Draw hypercolumn feature
% Arguments:
% #1 z-size
% #2 hc style
\newcommand{\drawHCfeature}[2]{%
   \psframe[style=#2](#1,1)%
}


==> diagrams/include/packages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LaTeX packages used by diagrams.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Fonts.
\usepackage{times}

% Math symbols.
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{accents}

% Pstricks.
\usepackage{pgffor}
\usepackage{pstricks}
\usepackage{pst-plot}
\usepackage{pst-text}
\usepackage{pst-node}
\usepackage{pst-tree}
\usepackage{pst-fill}
\usepackage{pst-3d}
\usepackage{pst-3dplot}
\usepackage{epsfig}

% Comments.
\usepackage{comment}


==> diagrams/include/styles.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Diagram styles.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% colors
\definecolor{faintgray}{rgb}{0.9,0.9,0.9}
\definecolor{lightgray}{rgb}{0.8,0.8,0.8}
\definecolor{darkgray}{rgb}{0.3,0.3,0.3}
\definecolor{nightgray}{rgb}{0.2,0.2,0.2}
\definecolor{darkgreen}{rgb}{0,0.75,0}
\definecolor{hotpink}{rgb}{0.95,0.08,0.82}

% blobs
\newpsstyle{encoderBlob}{
   linewidth = 0.5pt,
   fillstyle = solid,
   fillcolor = red,
   opacity   = 0.33
}
\newpsstyle{decoderBlob}{
   linewidth = 0.5pt,
   fillstyle = solid,
   fillcolor = blue,
   opacity   = 0.33
}
\newpsstyle{cnnBlob}{
   linewidth = 0.5pt,
   fillstyle = solid,
   fillcolor = gray,
   opacity   = 0.33
}

% hypercolumns
\newpsstyle{encoderHC}{
   linewidth = 1.0pt,
   linecolor = red
}
\newpsstyle{cnnHC}{
   linewidth = 1.0pt,
   linecolor = darkgreen
}
\newpsstyle{hcFeature}{
   linewidth = 0.5pt,
   fillstyle = solid,
   fillcolor = darkgreen,
   opacity   = 0.33
}

% connection arrows
\newpsstyle{hcArrow}{
   linewidth=3.0pt, linearc=5.0pt
}
\newpsstyle{auxArrow}{
   linewidth=4.0pt, linearc=5.0pt
}

% input/output arrows
\newpsstyle{ioArrow}{
   linewidth=1.5pt, linearc=5.0pt
}
\newpsstyle{hcPredArrow}{
   linewidth=1.0pt, linearc=1.0pt
}

% separators
\newpsstyle{sepline}{linecolor=black, linewidth=0.5pt, linestyle=dashed}


==> diagrams/include/styles_dark.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Diagram styles.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% colors
\definecolor{faintgray}{rgb}{0.9,0.9,0.9}
\definecolor{lightgray}{rgb}{0.8,0.8,0.8}
\definecolor{darkgray}{rgb}{0.3,0.3,0.3}
\definecolor{nightgray}{rgb}{0.2,0.2,0.2}
\definecolor{darkgreen}{rgb}{0,0.75,0}
\definecolor{hotpink}{rgb}{0.95,0.08,0.82}

% blobs
\newpsstyle{encoderBlob}{
   linewidth = 0.5pt,
   linecolor = lightgray,
   fillstyle = solid,
   fillcolor = red,
   opacity   = 0.50
}
\newpsstyle{decoderBlob}{
   linewidth = 0.5pt,
   linecolor = lightgray,
   fillstyle = solid,
   fillcolor = cyan,
   opacity   = 0.50
}
\newpsstyle{cnnBlob}{
   linewidth = 0.5pt,
   linecolor = lightgray,
   fillstyle = solid,
   fillcolor = gray,
   opacity   = 0.50
}

% hypercolumns
\newpsstyle{encoderHC}{
   linewidth = 1.0pt,
   linecolor = red
}
\newpsstyle{cnnHC}{
   linewidth = 1.0pt,
   linecolor = darkgreen
}
\newpsstyle{hcFeature}{
   linewidth = 0.5pt,
   linecolor = lightgray,
   fillstyle = solid,
   fillcolor = darkgreen,
   opacity   = 1.0
}

% connection arrows
\newpsstyle{hcArrow}{
   linecolor=white, linewidth=3.0pt, linearc=5.0pt
}
\newpsstyle{auxArrow}{
   linecolor=white, linewidth=4.0pt, linearc=5.0pt
}

% input/output arrows
\newpsstyle{ioArrow}{
   linecolor=white, linewidth=1.5pt, linearc=5.0pt
}
\newpsstyle{hcPredArrow}{
   linecolor=white, linewidth=1.0pt, linearc=1.0pt
}

% separators
\newpsstyle{sepline}{linecolor=white, linewidth=0.5pt, linestyle=dashed}


==> divsamp/Acknowledgments.tex <==
\section*{Acknowledgments}\label{sec:Acknowledgments} 

We gratefully acknowledge a gift of GPUs from
NVIDIA corporation. GS was partially supported by NSF
award 1409837.

==> include/label-reg/acknowledgements.tex <==
~\\
\noindent
{\small
\textbf{Acknowledgements.}  This work was in part supported by the DARPA
Lifelong Learning Machines program.}


==> include/label-reg/authors.tex <==
\author{%
Mohammadreza Mostajabi \and Michael Maire \and Gregory Shakhnarovich\\
\vspace{-0.028\linewidth}\and%
Toyota Technological Institute at Chicago\\
{\tt\small\{mostajabi,mmaire,greg\}@ttic.edu}%
\vspace{-0.01\linewidth}%
}


==> include/label-reg/fig_clusters.tex <==
\begin{figure}
   \begin{center}
      \vspace{5cm}
   \end{center}
   \caption{
      \textbf{Clusters in label space.}
   }
   \label{fig:clusters}
\end{figure}


==> include/label-reg/fig_densenet_201.tex <==
\begin{figure}
   \begin{center}
      \begin{scriptsize}
      \setlength\tabcolsep{4.5pt}
      \begin{tabular}{@{}c|c|c@{}}
      \footnotesize{Layers} & \footnotesize{DenseNet-121} & \footnotesize{DenseNet-201}\\
      \Hline
         & &\\[-7pt]
         Convolution
         &
            $\begin{bmatrix}
               7 \times 7\ \text{conv,}\\
               \text{stride 2}\\
            \end{bmatrix} \times 1$
         &
            $\begin{matrix}
               7 \times 7\ \text{conv,}\\
               \text{stride 2}\\
            \end{matrix}$
         \\[11pt]
      \hline
         Pooling &
            \multicolumn{2}{c}{$3 \times 3$ max pool, stride 2}\\
      \hline
         & &\\[-7pt]
         Dense Block (1)
         &
            $\begin{bmatrix}
               1 \times 1\ \text{conv}\\
               3 \times 3\ \text{conv}\\
            \end{bmatrix} \times 6$
         &
            $\begin{bmatrix}
               1 \times 1\ \text{conv}\\
               3 \times 3\ \text{conv}\\
            \end{bmatrix} \times 6$
         \\[5pt]
      \hline
         \multirow{2}{*}{Transition Layer (1)}
            & \multicolumn{2}{c}{$1 \times 1$ conv}\\
            \cline{2-3}
            & \multicolumn{2}{c}{$2 \times 2$ average pool, stride 2}\\
      \hline
         & &\\[-7pt]
         Dense Block (2)
         &
            $\begin{bmatrix}
               1 \times 1\ \text{conv} \\
               3 \times 3\ \text{conv}\\
            \end{bmatrix} \times 12$
         &
            $\begin{bmatrix}
               1 \times 1\ \text{conv} \\
               3 \times 3\ \text{conv}\\
            \end{bmatrix} \times 12$
         \\[5pt]
      \hline
         \\[-8pt]
         \multirow{2}{*}{Transition Layer (2)}
            & \multicolumn{2}{c}{$1 \times 1$ conv}\\
            \cline{2-3}
            & \multicolumn{2}{c}{$2 \times 2$ average pool, stride 2}\\
      \hline
         & &\\[-7pt]
         Dense Block (3)
         &
            $\begin{bmatrix}
               1 \times 1\ \text{conv} \\
               3 \times 3\ \text{conv}\\
            \end{bmatrix} \times 24$
         &
            $\begin{bmatrix}
               1 \times 1\ \text{conv} \\
               3 \times 3\ \text{conv}\\
            \end{bmatrix} \times 48$
         \\[5pt]
      \hline
         \multirow{2}{*}{Transition Layer (3)}
            & \multicolumn{2}{c}{$1 \times 1$ conv}\\
            \cline{2-3}
            & \multicolumn{2}{c}{$2 \times 2$ average pool, stride 2}\\
      \hline
         & &\\[-7pt]
         Dense Block (4)
         &
            $\begin{bmatrix}
               1 \times 1\ \text{conv}\\
               3 \times 3\ \text{conv}\\
            \end{bmatrix} \times 16$
         &
            $\begin{bmatrix}
               1 \times 1\ \text{conv}\\
               3 \times 3\ \text{conv}\\
            \end{bmatrix} \times 32$
         \\[5pt]
      \hline
      \end{tabular}
      \end{scriptsize}
      \vspace{0.01\linewidth}
      \caption{
         DenseNet architectural specifications.
      }
      \label{fig:densenet201}
   \end{center}
   \vspace{1\linewidth}
\end{figure}


==> include/label-reg/packages.tex <==
\usepackage{cvpr}
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{comment}
\usepackage{color}
\usepackage{rotating}
\usepackage{overpic}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{hhline}


==> include/label-reg/sec0_abstract.tex <==
We construct custom regularization functions for use in supervised training
of deep neural networks.  Our technique is applicable when the ground-truth
labels themselves exhibit internal structure; we derive a regularizer by
learning an autoencoder over the set of annotations.  Training thereby becomes
a two-phase procedure.  The first phase models labels with an autoencoder.
The second phase trains the actual network of interest by attaching an
auxiliary branch that must predict output via a hidden layer of the
autoencoder.  After training, we discard this auxiliary branch.

We experiment in the context of semantic segmentation, demonstrating this
regularization strategy leads to consistent accuracy boosts over baselines,
both when training from scratch, or in combination with ImageNet pretraining.
Gains are also consistent over different choices of convolutional network
architecture.  As our regularizer is discarded after training, our method has
zero cost at test time; the performance improvements are essentially free.
We are simply able to learn better network weights by building an abstract
model of the label space, and then training the network to understand this
abstraction alongside the original task.


==> label-reg/diagrams/include/blobs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Blobs.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Draw blob (back).
% Arguments:
% #1 x-size
% #2 y-size
% #3 z-size
% #4 style
\newcommand{\drawBlobBack}[4]{
   \ThreeDput[normal=1 0 0](0,0,0){
      \psframe[style=#4,fillcolor=white](#1,#2)}   % back
   \ThreeDput[normal=0 1 0](#3,#1,0){
      \psframe[style=#4,fillcolor=white](#3,#2)}   % far side
   \ThreeDput[normal=0 0 1](0,0,0){
      \psframe[style=#4,fillcolor=white](#3,#1)}   % bottom
}

% Draw blob (front).
% Arguments:
% #1 x-size
% #2 y-size
% #3 z-size
% #4 style
\newcommand{\drawBlobFront}[4]{
   \ThreeDput[normal=0 0 1](0,0,#2){
      \psframe[style=#4](#3,#1)}                   % top
   \ThreeDput[normal=0 1 0](#3,0,0){
      \psframe[style=#4](#3,#2)}                   % near side
   \ThreeDput[normal=1 0 0](#3,0,0){
      \psframe[style=#4](#1,#2)}                   % front
}

% Draw blob.
% Arguments:
% #1 x-size
% #2 y-size
% #3 z-size
% #4 style
\newcommand{\drawBlob}[4]{
   \drawBlobBack{#1}{#2}{#3}{#4}
   \drawBlobFront{#1}{#2}{#3}{#4}
}

% Draw blob with hypercolumn line.
% Arguments:
% #1 x-size
% #2 y-size
% #3 z-size
% #4 blob style
% #5 hc x-coord
% #6 hc y-coord
% #7 hc style
\newcommand{\drawBlobHC}[7]{
   \drawBlobBack{#1}{#2}{#3}{#4}                   % blob back
   \ThreeDput[normal=1 0 0](0,#5,#6){              % intersection back
      \psdot[dotsize=1.0](0,0)
   }
   \ThreeDput[normal=0 -1 0](0,#5,#6){             % hypercolumn
      \psline[style=#7]{-}(0,0)(#3,0)
   }
   \drawBlobFront{#1}{#2}{#3}{#4}                  % blob front
   \ThreeDput[normal=1 0 0](#3,#5,#6){             % intersection front
      \psdot[dotsize=1.0](0,0)
   }
}

% Draw hypercolumn feature
% Arguments:
% #1 z-size
% #2 hc style
\newcommand{\drawHCfeature}[2]{%
   \psframe[style=#2](#1,1)%
}


==> label-reg/diagrams/include/packages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LaTeX packages used by diagrams.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Fonts.
\usepackage{times}

% Math symbols.
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{accents}

% Pstricks.
\usepackage{pgffor}
\usepackage{pstricks}
\usepackage{pst-plot}
\usepackage{pst-text}
\usepackage{pst-node}
\usepackage{pst-tree}
\usepackage{pst-fill}
\usepackage{pst-3d}
\usepackage{pst-3dplot}
\usepackage{epsfig}

% Comments.
\usepackage{comment}


==> label-reg/diagrams/include/styles.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Diagram styles.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% colors
\definecolor{faintgray}{rgb}{0.9,0.9,0.9}
\definecolor{lightgray}{rgb}{0.8,0.8,0.8}
\definecolor{darkgray}{rgb}{0.3,0.3,0.3}
\definecolor{nightgray}{rgb}{0.2,0.2,0.2}
\definecolor{darkgreen}{rgb}{0,0.75,0}
\definecolor{hotpink}{rgb}{0.95,0.08,0.82}

% blobs
\newpsstyle{encoderBlob}{
   linewidth = 0.5pt,
   fillstyle = solid,
   fillcolor = red,
   opacity   = 0.33
}
\newpsstyle{decoderBlob}{
   linewidth = 0.5pt,
   fillstyle = solid,
   fillcolor = blue,
   opacity   = 0.33
}
\newpsstyle{cnnBlob}{
   linewidth = 0.5pt,
   fillstyle = solid,
   fillcolor = gray,
   opacity   = 0.33
}

% hypercolumns
\newpsstyle{encoderHC}{
   linewidth = 1.0pt,
   linecolor = red
}
\newpsstyle{cnnHC}{
   linewidth = 1.0pt,
   linecolor = darkgreen
}
\newpsstyle{hcFeature}{
   linewidth = 0.5pt,
   fillstyle = solid,
   fillcolor = darkgreen,
   opacity   = 0.33
}

% connection arrows
\newpsstyle{hcArrow}{
   linewidth=3.0pt, linearc=5.0pt
}
\newpsstyle{auxArrow}{
   linewidth=4.0pt, linearc=5.0pt
}

% input/output arrows
\newpsstyle{ioArrow}{
   linewidth=1.5pt, linearc=5.0pt
}
\newpsstyle{hcPredArrow}{
   linewidth=1.0pt, linearc=1.0pt
}

% separators
\newpsstyle{sepline}{linecolor=black, linewidth=0.5pt, linestyle=dashed}


==> label-reg/diagrams/include/styles_dark.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Diagram styles.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% colors
\definecolor{faintgray}{rgb}{0.9,0.9,0.9}
\definecolor{lightgray}{rgb}{0.8,0.8,0.8}
\definecolor{darkgray}{rgb}{0.3,0.3,0.3}
\definecolor{nightgray}{rgb}{0.2,0.2,0.2}
\definecolor{darkgreen}{rgb}{0,0.75,0}
\definecolor{hotpink}{rgb}{0.95,0.08,0.82}

% blobs
\newpsstyle{encoderBlob}{
   linewidth = 0.5pt,
   linecolor = lightgray,
   fillstyle = solid,
   fillcolor = red,
   opacity   = 0.50
}
\newpsstyle{decoderBlob}{
   linewidth = 0.5pt,
   linecolor = lightgray,
   fillstyle = solid,
   fillcolor = cyan,
   opacity   = 0.50
}
\newpsstyle{cnnBlob}{
   linewidth = 0.5pt,
   linecolor = lightgray,
   fillstyle = solid,
   fillcolor = gray,
   opacity   = 0.50
}

% hypercolumns
\newpsstyle{encoderHC}{
   linewidth = 1.0pt,
   linecolor = red
}
\newpsstyle{cnnHC}{
   linewidth = 1.0pt,
   linecolor = darkgreen
}
\newpsstyle{hcFeature}{
   linewidth = 0.5pt,
   linecolor = lightgray,
   fillstyle = solid,
   fillcolor = darkgreen,
   opacity   = 1.0
}

% connection arrows
\newpsstyle{hcArrow}{
   linecolor=white, linewidth=3.0pt, linearc=5.0pt
}
\newpsstyle{auxArrow}{
   linecolor=white, linewidth=4.0pt, linearc=5.0pt
}

% input/output arrows
\newpsstyle{ioArrow}{
   linecolor=white, linewidth=1.5pt, linearc=5.0pt
}
\newpsstyle{hcPredArrow}{
   linecolor=white, linewidth=1.0pt, linearc=1.0pt
}

% separators
\newpsstyle{sepline}{linecolor=white, linewidth=0.5pt, linestyle=dashed}


==> notation.tex <==
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\mathA}{\mathbb{A}}
\newcommand{\mathB}{\mathbb{B}}
\newcommand{\mathC}{\mathbb{C}}
\newcommand{\mathD}{\mathbb{D}}
\newcommand{\mathE}{\mathbb{E}}
\newcommand{\mathF}{\mathbb{F}}
\newcommand{\mathG}{\mathbb{G}}
\newcommand{\mathH}{\mathbb{H}}
\newcommand{\mathI}{\mathbb{I}}
\newcommand{\mathJ}{\mathbb{J}}
\newcommand{\mathK}{\mathbb{K}}
\newcommand{\mathL}{\mathbb{L}}
\newcommand{\mathM}{\mathbb{M}}
\newcommand{\mathN}{\mathbb{N}}
\newcommand{\mathO}{\mathbb{O}}
\newcommand{\mathP}{\mathbb{P}}
\newcommand{\mathQ}{\mathbb{Q}}
\newcommand{\mathR}{\mathbb{R}}
\newcommand{\mathS}{\mathbb{S}}
\newcommand{\mathT}{\mathbb{T}}
\newcommand{\mathU}{\mathbb{U}}
\newcommand{\mathV}{\mathbb{V}}
\newcommand{\mathW}{\mathbb{W}}
\newcommand{\mathX}{\mathbb{X}}
\newcommand{\mathY}{\mathbb{Y}}
\newcommand{\mathZ}{\mathbb{Z}}

\newcommand{\vecA}{\mathbf{A}}
\newcommand{\vecB}{\mathbf{B}}
\newcommand{\vecC}{\mathbf{C}}
\newcommand{\vecD}{\mathbf{D}}
\newcommand{\vecE}{\mathbf{E}}
\newcommand{\vecF}{\mathbf{F}}
\newcommand{\vecG}{\mathbf{G}}
\newcommand{\vecH}{\mathbf{H}}
\newcommand{\vecI}{\mathbf{I}}
\newcommand{\vecJ}{\mathbf{J}}
\newcommand{\vecK}{\mathbf{K}}
\newcommand{\vecL}{\mathbf{L}}
\newcommand{\vecM}{\mathbf{M}}
\newcommand{\vecN}{\mathbf{N}}
\newcommand{\vecO}{\mathbf{O}}
\newcommand{\vecP}{\mathbf{P}}
\newcommand{\vecQ}{\mathbf{Q}}
\newcommand{\vecR}{\mathbf{R}}
\newcommand{\vecS}{\mathbf{S}}
\newcommand{\vecT}{\mathbf{T}}
\newcommand{\vecU}{\mathbf{U}}
\newcommand{\vecV}{\mathbf{V}}
\newcommand{\vecW}{\mathbf{W}}
\newcommand{\vecX}{\mathbf{X}}
\newcommand{\vecY}{\mathbf{Y}}
\newcommand{\vecZ}{\mathbf{Z}}
\newcommand{\vecAlpha}{\boldsymbol{\alpha}}
\newcommand{\vecBeta}{\boldsymbol{\beta}}
\newcommand{\vecGamma}{\boldsymbol{\gamma}}
\newcommand{\vecLambda}{\boldsymbol{\lambda}}
\newcommand{\vecDelta}{\boldsymbol{\Delta}}
\newcommand{\vecdelta}{\boldsymbol{\delta}}
\newcommand{\vecphi}{\boldsymbol{\phi}}
\newcommand{\vectheta}{\boldsymbol{\theta}}

\newcommand{\veca}{\mathbf{a}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\vecc}{\mathbf{c}}
\newcommand{\vecd}{\mathbf{d}}
\newcommand{\vece}{\mathbf{e}}
\newcommand{\vecf}{\mathbf{f}}
\newcommand{\vecg}{\mathbf{g}}
\newcommand{\vech}{\mathbf{h}}
\newcommand{\veci}{\mathbf{i}}
\newcommand{\vecj}{\mathbf{j}}
\newcommand{\veck}{\mathbf{k}}
\newcommand{\vecl}{\mathbf{l}}
\newcommand{\vecm}{\mathbf{m}}
\newcommand{\vecn}{\mathbf{n}}
\newcommand{\veco}{\mathbf{o}}
\newcommand{\vecp}{\mathbf{p}}
\newcommand{\vecq}{\mathbf{q}}
\newcommand{\vecr}{\mathbf{r}}
\newcommand{\vecs}{\mathbf{s}}
\newcommand{\vect}{\mathbf{t}}
\newcommand{\vecu}{\mathbf{u}}
\newcommand{\vecv}{\mathbf{v}}
\newcommand{\vecw}{\mathbf{w}}
\newcommand{\vecx}{\mathbf{x}}
\newcommand{\vecy}{\mathbf{y}}
\newcommand{\vecz}{\mathbf{z}}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\cov}{Cov}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\length}{len}

\newcommand{\removed}[1]{}
\newcommand{\defeq}{\stackrel{\text{def}}{=}}
\newcommand{\one}[1]{\left[\!\left[ #1 \right]\!\right]}
\newcommand{\argmin}[1]{\underset{#1}{\mathrm{argmin}} \:}
\newcommand{\argmax}[1]{\underset{#1}{\mathrm{argmax}} \:}
\newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\E}[1]{{\mathbb{E}\left[{#1}\right]}}
\newcommand{\hE}[1]{{\mathbb{\hat{E}}\left[{#1}\right]}}
\newcommand{\Ep}[2]{{\mathbb{E}_{#1}\left[{#2}\right]}}
\newcommand{\hinge}[1]{[#1]_+}
\newcommand{\norm}[1]{\left\lVert{#1}\right\rVert}
\newcommand{\abs}[1]{{\left\lvert{#1}\right\rvert}}
\newcommand{\margin}{\text{margin}}

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\pr}[2]{{\mathbb{P}_{#1}\left[{#2}\right]}}

\newcommand{\net}{\text{net}}
\newcommand{\eps}{\epsilon}
\newcommand{\tW}{\widetilde{W}}
\newcommand{\In}{\text{in}}
\newcommand{\Out}{\text{out}}
\newcommand{\Win}{\vecW_{\text{in}}}
\newcommand{\Wout}{\vecW_{\text{out}}}
\newcommand{\Wrec}{\vecW_{\text{rec}}}
\newcommand{\relu}{\sigma_{\textsc{relu}}}
\newcommand{\err}{Err}
\newcommand{\error}{\epsilon}
\newcommand{\hatD}{\widehat{D}}
\newcommand{\hatL}{\hat{L}}
\newcommand{\hatl}{\hat{\ell}}

\newcommand{\vin}{v_{\textrm{in}}}
\newcommand{\vout}{v_{\textrm{out}}}
\newcommand{\layer}{\text{layer}}
\newcommand{\gnorm}[1]{\norm{#1}}
\newcommand{\pathr}{\phi}
\newcommand{\DAG}{\text{DAG}}
\newcommand{\convexnn}{\nu}
\newcommand{\nout}{n_\text{out}}
\newcommand{\nin}{n_\text{in}}
\newcommand{\netdepth}{d}
\newcommand{\netwidth}{H}
\newcommand{\nparam}{n_{\text{param}}}
